Measuring Statistical Evidence: A Short Report

This short text tried to establish a big picture of what evidential statistics is about and how an ideal inference method should behave. Moreover, by examining shortcomings of some of the currently used methods for measuring evidence and utilizing some intuitive principles, we motivated the Relative Belief Ratio as the primary method of characterizing statistical evidence. Number of topics has been omitted for the interest of this text and the reader is strongly advised to refer to (Evans, 2015) as the primary source for further readings of the subject.

==> ch0.tex <==
\chapter*{Introduction}

What is statistics (short history)
- base problem in stats
- inference setup (need for estimation or hypothesis testing and accuracy stuff.)

assessing the error in estimation and hypothesis assessment relation

desirable things for theory of statistics as a way of reasoning : 
- falsifiability 
- settle subjectivity and objectivity (model, data, scientist)
- need for logical theory
- ideally free of arbitrary choices

evidential vs decision theoric school of thought
    utility, falsifiability of loss function, paradoxes, problems with maximizing expected utility (phl)




mathematical statistics vs stats

stats is not magic. give me the ingredients and draw inference. 

mention borel paradox and say that we are ommiting issues that its because underspecification of the problem 

ignoring rejection trials due to being decision theoric. 


decision theory : british and american school of stats and a new classification.
